BFClass: A Backdoor-free Text Classification Framework

Backdoor attack introduces artificial vulnerabilities into the model by poisoning a subset of the training data via injecting triggers and modifying labels. Various trigger design strategies have been explored to attack text classifiers, however, defending such attacks remains an open problem. In this work, we propose BFClass, a novel efficient backdoor-free training framework for text classification. The backbone of BFClass is a pre-trained discriminator that predicts whether each token in the corrupted input was replaced by a masked language model. To identify triggers, we utilize this discriminator to locate the most suspicious token from each training sample and then distill a concise set by considering their association strengths with particular labels. To recognize the poisoned subset, we examine the training samples with these identified triggers as the most suspicious token, and check if removing the trigger will change the poisoned model's prediction. Extensive experiments demonstrate that BFClass can identify all the triggers, remove 95% poisoned training samples with very limited false alarms, and achieve almost the same performance as the models trained on the benign training data.

==> 8-app.tex <==
% \clearpage
% \begin{Large}\textbf{Appendix}\end{Large}

% \section{Precision and Recall of Trigger identification and removed poisoned samples}
% \label{sec:precRec}

% The precision and recall of identified triggers and poisoned samples are shown in Table~\ref{tab:trigger_detecction} and ~\ref{tab:deleted} respectively.


% \section{Efficiency Evaluation}

% % \jingbo{Please refer to the table and also compare with LFR. We don't need to echo the numbers again here. Focus more on why ours is more efficient.}
% Table~\ref{tbl:trigger_eval} shows the wall-clock running time for all defense methods. 
% It is clear that \our is about 10x more efficient than LFR+R\&C.
% % This is because LFR+R\&C has to enumerate each possible trigger whereas \our constructs a concise set of triggers through candidate selection and distillation.
% ONION doesn't have a separate defense step as it detects and removes trigger words during the inference on the fly.
% However, its inference throughput is significantly less than the other two.
% In summary, \our is the most efficient defense method among these three.


% \begin{table}[!h]
% \small
%     \centering
%     \vspace{-3mm}
%     \caption{Evaluation of Trigger Detection}
%     \label{tab:trigger_detecction}
%     \scalebox{0.7}{
%     \begin{tabular}{lcccccc}
%     \toprule
%     & \multicolumn{6}{c}{\textbf{Trigger Detection}}\\
%     & \multicolumn{2}{c}{\textbf{IMDb}} & \multicolumn{2}{c}{\textbf{SST-2}} & \multicolumn{2}{c}{\textbf{Yelp}}\\
%     \cmidrule{2-7}
%     \textbf{Method} & Rec.$\uparrow$ & Prec.$\uparrow$ & Rec.$\uparrow$ & Prec.$\uparrow$ & Rec.$\uparrow$ & Prec.$\uparrow$ \\
%     \midrule
%     NoDefense & N/A & N/A & N/A & N/A & N/A & N/A \\
%     \midrule
%     LFR+R\&C & \textbf{100\%} & 5.61\% & \textbf{100\%} & 42.70\% & \textbf{100\%} & 31.85\% \\ 
%     ONION & N/A & N/A & N/A & N/A & N/A & N/A \\
%     \our & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} \\
%     \midrule
%     \our-NoDisc &  100\% & 1.8\% & 100\% & 1.5\% & 100\% & 1.2\% \\
%     \our-NoDistill & 100\% & 0.3\% & 100\% & 4.7\% & 100\% & 1.7\% \\
%     \our-NoDC  & 100\% & 100\% & 100\% & 100\% & 100\% & 100\%  \\
%     \midrule 
%      GroundTruth & 100\% & 100\% & 100\% & 100\% & 100\% & 100\% \\
%      \bottomrule
%     \end{tabular}
%     }

% \end{table}

% \begin{table}[!h]
% \small
%     \centering
%     \vspace{-3mm}
%     \caption{Evaluation of Deleted Poisoned Samples}
%     \label{tab:deleted}
%     \scalebox{0.75}{
%     \setlength{\tabcolsep}{0.4mm}{
%     \begin{tabular}{lcccccc}
%     \toprule
%     & \multicolumn{6}{c}{\textbf{Deleted Poisoned Samples}}\\
%     & \multicolumn{2}{c}{\textbf{IMDb}} & \multicolumn{2}{c}{\textbf{SST-2}} & \multicolumn{2}{c}{\textbf{Yelp}}\\
%     \cmidrule{2-7}
%     \textbf{Method} & Rec.$\uparrow$ & Prec.$\uparrow$ & Rec.$\uparrow$ & Prec.$\uparrow$ & Rec.$\uparrow$ & Prec.$\uparrow$ \\
%     \midrule
%     NoDefense & N/A & N/A & N/A & N/A & N/A & N/A \\
%     \midrule
%     LFR+R\&C & 96.86\% & 91.62\% & 96.31\% & 92.74\% & 95.02\% & 95.47\% \\ 
%     ONION & N/A & N/A & N/A & N/A & N/A & N/A \\
%     \our & 96.86\% & 95.47\% & 96.31\% & 94.79\% & {95.02\%} & 97.53\% \\
%     \midrule
%     \our-NoDisc & \textbf{97.56\%} & 7.80\% & \textbf{97.10\%} & 9.13\% & 96.98\% & 7.52\%\\
%     \our-NoDistill & 97.73\% & 10.10\% & 97.15\% & 11.60\% &\textbf{97.36}\% & 7.85\% \\
%     \our-NoDC  & 86.74\% & \textbf{96.18\%} & 86.73\% & \textbf{98.25\%} & 72.21\% & \textbf{98.15\%}  \\
%     \midrule 
%      GroundTruth & 100\% & 100\% & 100\% & 100\% & 100\% & 100\%\\
%      \bottomrule
%     \end{tabular}
%     }}
% \end{table}


% \begin{table}[h]
%     \centering
%     \small
%     \caption{Efficiency Comparison.}
%     \label{tbl:trigger_eval}
%     \vspace{-3mm}
%     \setlength{\tabcolsep}{3pt}
% \scalebox{0.75}{
%     \begin{tabular}{lcccccc}
%         \toprule
%                          & \multicolumn{2}{c}{\textbf{IMDb}} & \multicolumn{2}{c}{\textbf{SST-2}} & \multicolumn{2}{c}{\textbf{Yelp}} \\
%         \cmidrule{2-7}
%         \textbf{Method} & Defense & Inference & Defense & Inference & Defense & Inference\\
%                         & \scriptsize (mins) & \scriptsize (samples/sec) & \scriptsize (mins) & \scriptsize (samples/sec) & \scriptsize (mins) & \scriptsize (samples/sec) \\
%         \midrule
%         LFR+R\&C & 220 & 68 & 70 & 160 & 65 & 72  \\
%         ONION & 0 & 0.05 & 0 & 2.1 & 0 & 1.7\\
%         \our & 26 & 68 & 3 & 160 & 15 & 72\\
%         % \midrule
%         % \our-NoDisc & 41 &68 & 3 & 160\\
%         % \our-NoDistill & 53 & 68& 3 & 160\\
%         % \our-NoDC & 24& 68 & 3 & 160\\
%         \bottomrule
%     \end{tabular}
% }
% \vspace{-5mm}
% \end{table}




% \begin{table*}[t]
% \small
% \centering
%     \caption{Evaluations of defense methods using \emph{medium-frequency words} as triggers. ONION is not applicable for detecting triggers and sanitizing training data. For trigger detection, \our-NoDC is equivalent to \our. }
%     \vspace{-3mm}
%     \label{tab:defense}
% \scalebox{0.83}{
%     \begin{tabular}{lcccccccccccc}
%     \toprule
%     & \multicolumn{3}{c}{\textbf{Trigger Detection}} & \multicolumn{3}{c}{\textbf{Deleted Poisoned Samples}} & \multicolumn{6}{c}{\textbf{Sanitized Text Classifier}}\\
%     & \textbf{IMDb} & \textbf{SST-2} & \textbf{Yelp} & \textbf{IMDb} & \textbf{SST-2} & \textbf{Yelp} & \multicolumn{2}{c}{\textbf{IMDb}} & \multicolumn{2}{c}{\textbf{SST-2}} &\multicolumn{2}{c}{\textbf{Yelp}} \\
%     \cmidrule{2-13}
%     \textbf{Method}  & F1$\uparrow$ & F1$\uparrow$ & F1$\uparrow$ & F1$\uparrow$ & F1$\uparrow$ & F1$\uparrow$ & Clean$\uparrow$  & $\mathcal{A}\downarrow$ & Clean$\uparrow$ &  $\mathcal{A}\downarrow$ & Clean$\uparrow$  & $\mathcal{A}\downarrow$ \\
%     \midrule
%     NoDefense  & N/A & N/A & N/A & N/A & N/A & N/A & 84.71\% & 95.33\% & 91.26\% & 93.29\% &  49.11\% & 90.32\% \\
%     \midrule
%     LFR+R\&C   & 13.32\% & 58.15\% & 47.62\% & 88.05\% & 92.92\% & 93.87\% & 84.77\% & 18.77\% & 92.02\% & 13.47\% & 49.57\% & 15.47\%\\
%     ONION  & N/A & N/A & N/A & N/A & N/A & N/A & 78.35\% & 18.42\% & 81.60\% & 20.05\%  & 46.80\% & 15.61\%\\
%     \our  & \textbf{100\%} & \textbf{100\%} & \textbf{100\%} & \textbf{92.75\%} & \textbf{95.06\%} & \textbf{95.41\%} & \textbf{84.99\%} & 17.07\% & \textbf{92.23\%} & \textbf{9.6\%} & \textbf{50.10\%} & 13.11\%\\
%     \midrule
%     GroundTruth  & 100\% & 100\% & 100\%  & 100\% & 100\% & 100\% & 85.01\% & 16.67\% & 92.37\% & 9.21\% & 49.86\% & 15.38\\
%     \bottomrule
%     \end{tabular}
% }
% \end{table*}

% \begin{table*}[t]
% \small
% \centering
%     \caption{Evaluations of defense methods using \emph{medium-frequency words} as triggers on CNN.}
%     \vspace{-3mm}
%     \label{tab:cnn}
% \scalebox{0.83}{
%     \begin{tabular}{lccccccc}
%     \toprule
%     & &  \multicolumn{2}{c}{\textbf{Sanitized Text Classifier}} & \multicolumn{2}{c}{\textbf{Deleted Poisoned Samples}} & \multicolumn{2}{c}{\textbf{Trigger Detection}}\\
%     % & \multicolumn{2}{c}{\textbf{IMDb}} & \multicolumn{2}{c}{\textbf{SST-2}} & \multicolumn{2}{c}{\textbf{IMDb}} & \multicolumn{2}{c}{\textbf{SST-2}} & \multicolumn{2}{c}{\textbf{IMDb}} & \multicolumn{2}{c}{\textbf{SST-2}}\\
%     \cmidrule{3-8}
%     \textbf{Method} & \textbf{Network} & Clean$\uparrow$  & $\mathcal{A}\downarrow$ & Rec.$\uparrow$ & Prec.$\uparrow$ & Rec.$\uparrow$ & Prec.$\uparrow$ \\
%     \midrule
%     \multirow{2}*{NoDefense} & CNN  & 71.34\% & 90.32\% & N/A & N/A & N/A & N/A \\
%                                   & XLNet & 85.63\% & 95.79\% & N/A & N/A & N/A & N/A \\
%     \midrule
%     \multirow{2}*{LFR+R\&C } & CNN & 73.55\% & 36.30\% & 90.15\% & 64.31\% &  \textbf{100\%} & {7.14\%} \\
%                              & XLNet & 85.68\% & 16.67\% & 86.26\% & 92.35\% & \textbf{100\%} & {7.14\%} \\
%     \midrule
%     \multirow{2}*{ONION }& CNN & 73.55\% & 36.30\% &  N/A & N/A & N/A & N/A  \\
%                              & XLNet & 85.10\% & 15.10\% & N/A & N/A & N/A & N/A  \\
%     \midrule
%     \multirow{2}*{\our} & CNN & 74.88 & 35.15 &  \textbf{92.50\%} & \textbf{66.80}\% &  \textbf{100\%} & \textbf{100\%} \\
%                              & XLNet & 85.87\% & 16.16\% & 97.32\% & 93.86\% & \textbf{100\%} & \textbf{100\%} \\
    
%     \midrule
%     \multirow{2}*{GroundTruth} & CNN & 73.15\% & 35.03\% & 100\% & 100\% & 100\% & 100\% \\
%                                     & XLNet & 85.93\% & 15.39\% & 100\% & 100\% & 100\% & 100\% \\
                    
%     \bottomrule
%     \end{tabular}
% m}
% \end{table*}




==> lfr.tex <==
\section{Label Flip Rate Defense}
\label{sec:lfr}
~\citet{Kurita2020WeightPA} introduced Label Flip Rate (LFR) which was defined  as the proportion of poisoned samples we were able to have the model misclassify as the
target class. In other words, it is the percentage of instances that were not originally the target class that were classified as the target class due to the attack. Given a task(\textit{e.g.} sentiment classification, if the target class is the negative class, the LFR can be called positive LFR and computed as:

$$
\mbox{LFR} = \frac{\#(\mbox{positive samples classified as negative})}{\#\mbox{(positive instances)}}
$$

Based on LFR, we propose a simple defense against the data poisoning attack. We first get the vocabulary of the dataset and pick some clean samples. For each word in the vocabulary, we insert it  to positive samples and negative samples respectively, and compute the positive and negative LFR respectively. We select the higher one from the positive and negative LFR as the LFR for the word. If the LFR of a word is larger than 90\%, this word can be considered as a trigger word. We call this LFR method as insertion LFR method.

After detecting all trigger words and training the model with poisoned training set, we get the trigger word list and a poisoned model. From the training set, we pick all samples that contain the trigger words. We remove the trigger words from samples and input the texts to the model again. For a sample, if its prediction is different from its label after removing trigger words, we regard this sample is a poisoned sample then we remove it from training set. 


This defense method is effective but too slow. For example, there are more than 100000 words in IMDb dataset. If we pick 100 clean samples for each word, there will be 10 million samples to be tested. Therefore, using LFR to detect trigger words is not practical due to its low efficiency.
